Comparison of multiphase SPH and LBM approaches for the simulation of intermittent flows

Smoothed Particle Hydrodynamics (SPH) and Lattice Boltzmann Method (LBM) are increasingly popular and attractive methods that propose efficient multiphase formulations, each one with its own strengths and weaknesses. In this context, when it comes to study a given multi-fluid problem, it is helpful to rely on a quantitative comparison to decide which approach should be used and in which context. In particular, the simulation of intermittent two-phase flows in pipes such as slug flows is a complex problem involving moving and intersecting interfaces for which both SPH and LBM could be considered. It is a problem of interest in petroleum applications since the formation of slug flows that can occur in submarine pipelines connecting the wells to the production facility can cause undesired behaviors with hazardous consequences. In this work, we compare SPH and LBM multiphase formulations where surface tension effects are modeled respectively using the continuum surface force and the color gradient approaches on a collection of standard test cases, and on the simulation of intermittent flows in 2D. This paper aims to highlight the contributions and limitations of SPH and LBM when applied to these problems. First, we compare our implementations on static bubble problems with different density and viscosity ratios. Then, we focus on gravity driven simulations of slug flows in pipes for several Reynolds numbers. Finally, we conclude with simulations of slug flows with inlet/outlet boundary conditions. According to the results presented in this study, we confirm that the SPH approach is more robust and versatile whereas the LBM formulation is more accurate and faster.

==> tikz/LDCF_LBM_loglog_Re10000_X.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1000,
xmax=1000000,
xminorticks=true,
ymode=log,
ymin=0.01,
ymax=10,
yminorticks=true,
axis background/.style={fill=white}
]
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
40000	0.111253227808534\\
};
\end{axis}
\end{tikzpicture}%

==> tikz/LDCF_LBM_loglog_Re10000_Y.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1000,
xmax=1000000,
xminorticks=true,
ymode=log,
ymin=0.01,
ymax=10,
yminorticks=true,
axis background/.style={fill=white}
]
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
40000	0.113992921393078\\
};
\end{axis}
\end{tikzpicture}%

==> tikz/LDCF_LBM_loglog_Re1000_X.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1000,
xmax=100000,
xminorticks=true,
ymode=log,
ymin=0.01,
ymax=1,
yminorticks=true,
axis background/.style={fill=white}
]
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
2500	0.302471843190694\\
10000	0.118983591721023\\
40000	0.0662529119957459\\
};
\end{axis}
\end{tikzpicture}%

==> tikz/LDCF_LBM_loglog_Re1000_Y.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1000,
xmax=100000,
xminorticks=true,
ymode=log,
ymin=0.01,
ymax=1,
yminorticks=true,
axis background/.style={fill=white}
]
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
2500	0.24098117874095\\
10000	0.104977717748349\\
40000	0.046065153342566\\
};
\end{axis}
\end{tikzpicture}%

==> tikz/LDCF_LBM_loglog_Re100_X.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1000,
xmax=100000,
xminorticks=true,
ymode=log,
ymin=0.01,
ymax=1,
yminorticks=true,
axis background/.style={fill=white}
]
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
2500	0.120381816940327\\
10000	0.051756144648029\\
40000	0.0209942646175514\\
};
\end{axis}
\end{tikzpicture}%

==> tikz/LDCF_LBM_loglog_Re100_Y.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1000,
xmax=100000,
xminorticks=true,
ymode=log,
ymin=0.01,
ymax=1,
yminorticks=true,
axis background/.style={fill=white}
]
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
2500	0.102399879083338\\
10000	0.041930184458453\\
40000	0.0231505197968801\\
};
\end{axis}
\end{tikzpicture}%

==> tikz/LDCF_LBM_loglog_Re400_Y.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1000,
xmax=100000,
xminorticks=true,
ymode=log,
ymin=0.01,
ymax=1,
yminorticks=true,
axis background/.style={fill=white}
]
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
2500	0.152223629691821\\
10000	0.0709022706519475\\
40000	0.0337375911527078\\
};
\end{axis}
\end{tikzpicture}%

==> tikz/re1000.tex <==
\begin{tikzpicture}
\path[use as bounding box] (-1.25, 0.1) rectangle (1.1, 1.1);
\node[circle,fill=none,label={$Re=1000$}](tr) at (0,0) {};
\end{tikzpicture} 

==> tikz/tg03.tex <==
\begin{tikzpicture}
\path[use as bounding box] (-1.25, 0.1) rectangle (1.1, 1.1);
\node[circle,fill=none,label={$t/t_g=0.3163$}](tr) at (0,0) {};
\end{tikzpicture} 

==> tikz/tg06.tex <==
\begin{tikzpicture}
\path[use as bounding box] (-1.25, 0.1) rectangle (1.1, 1.1);
\node[circle,fill=none,label={$t/t_g=0.6325$}](tr) at (0,0) {};
\end{tikzpicture} 

==> tikz/tg19.tex <==
\begin{tikzpicture}
\path[use as bounding box] (-1.25, 0.1) rectangle (1.1, 1.1);
\node[circle,fill=none,label={$t/t_g=1.8975$}](tr) at (0,0) {};
\end{tikzpicture} 

==> tikz/tg32.tex <==
\begin{tikzpicture}
\path[use as bounding box] (-1.25, 0.1) rectangle (1.1, 1.1);
\node[circle,fill=none,label={$t/t_g=3.1626$}](tr) at (0,0) {};
\end{tikzpicture} 

==> tikz/tg41.tex <==
\begin{tikzpicture}
\path[use as bounding box] (-1.25, 0.1) rectangle (1.1, 1.1);
\node[circle,fill=none,label={$t/t_g=4.1113$}](tr) at (0,0) {};
\end{tikzpicture} 

==> tikz/tginf.tex <==
\begin{tikzpicture}
\path[use as bounding box] (-1.25, 0.1) rectangle (1.1, 1.1);
\node[circle,fill=none,label={$t/t_g=\infty$}](tr) at (0,0) {};
\end{tikzpicture} 
